Intensional view of General Single Processor Operating Systems

Operating systems are currently viewed ostensively. As a result they mean different things to different people. The ostensive character makes it is hard to understand OSes formally. An intensional view can enable better formal work, and also offer constructive support for some important problems, e.g. OS architecture. This work argues for an intensional view of operating systems. It proposes to overcome the current ostensive view by defining an OS based on formal models of computation, and also introduces some principles. Together these are used to develop a framework of algorithms of single processor OS structure using an approach similar to function level programming. In this abridged paper we illustrate the essential approach, discuss some advantages and limitations and point out some future possibilities.

==> Makefile <==
#
# Paper on Operating Systems
#
# Rewrite #5
#
# Start: October 29, 2012.
# End: March 31, 2013.     SOSP'13
# End: May 27, 2013.       TRIOS notes.
# End: August 02, 2013.    arXiv
#
### Directory Structure
TOP=$(shell pwd)
SRCDIR=$(TOP)
BLDDIR=$(TOP)/build
OUTDIR=$(TOP)
IMGDIR=$(TOP)
FIGDIR=$(IMGDIR)
EPSDIR=$(IMGDIR)
IMGOUTDIR=$(IMGDIR)
RELSRCDIR=.
RELEPSDIR=.

### Commands and options (if any)
#LATEX=pdflatex
TODAY=$(shell date +%d-%m-%Y-%H-%M-%S)
DVIPS=dvips
LATEX=latex
DVIPDF=dvipdf
PS2PDF=ps2pdf
BIBTEX=bibtex
LATEXOPTS=-interaction=batchmode -output-directory=$(BLDDIR)

# For arXiv
ARXIVNAME=intensional-view-of-oses
ARXIVBIBFILE=$(SRCDIR)/refs.bib
ARXIVSOURCES=$(SRCDIR)/$(ARXIVNAME).tex

ARXIVRELBIBFILE=$(RELSRCDIR)/refs.bib
ARXIVRELSOURCES=$(RELSRCDIR)/$(ARXIVNAME).tex    \
	        $(ARXIVRELBIBFILE)
ARXIVRELMAKEFILE=Makefile

ARXIVMAINTEX=$(BLDDIR)/$(ARXIVNAME).tex

ARXIVDVIOUT=$(ARXIVNAME).dvi
ARXIVPSOUT=$(ARXIVNAME).ps
ARXIVPDFOUT=$(ARXIVNAME).pdf

ARXIVAUX=$(ARXIVNAME).aux
ARXIVTOC=$(ARXIVNAME).toc
ARXIVLOG=$(ARXIVNAME).log
ARXIVFIG=$(ARXIVNAME).lof
ARXIVTAB=$(ARXIVNAME).lot
ARXIVTGZ=$(ARXIVNAME)-$(TODAY).tgz

ALLTGZ=arxivsrc-$(TODAY).tgz

# Targets
default: all

all: cls

cls: arxiv
	@/bin/rm -rf               \
	   $(OUTDIR)/$(ARXIVPSOUT) \
	   $(BLDDIR)
	@echo "Done."

tarall: arxivtar

# ARXIV Target
arxiv: outdirexist $(ARXIVPDFOUT)
	@echo -n "-> Moving `basename $(ARXIVPDFOUT)`"   && \
	echo -n " to `basename $(OUTDIR)`/ ... "         && \
	cd $(BLDDIR)                                     && \
	mv -f $(ARXIVPDFOUT) $(OUTDIR)                   && \
	cd $(TOP)

$(ARXIVPDFOUT): $(ARXIVPSOUT)
	@echo -n "-> Generating PDF from `basename $(ARXIVPSOUT)`  ... "  && \
	cd $(BLDDIR)                                                      && \
	$(PS2PDF) $(ARXIVPSOUT) $(ARXIVPDFOUT) > /dev/null 2>&1           && \
	/bin/rm $(ARXIVPSOUT)                                             && \
	cd $(TOP)                                                         && \
	echo "Done."

$(ARXIVPSOUT): $(ARXIVDVIOUT)
	@echo -n "-> Generating PS  from `basename $(ARXIVDVIOUT)` ... "  && \
	cd $(BLDDIR)                                                      && \
	$(DVIPS) -q $(ARXIVDVIOUT) -o $(ARXIVPSOUT)                       && \
	cd $(TOP)                                                         && \
	echo "Done."

$(ARXIVDVIOUT): blddirexist $(ARXIVSOURCES)
	@echo -n "-> Generating DVI from `basename $(ARXIVMAINTEX)` ... "  && \
	cp $(ARXIVSOURCES) $(BLDDIR)                                       && \
	cp $(SRCDIR)/*.eps $(BLDDIR)                                       && \
	cd $(BLDDIR)                                                       && \
	$(LATEX)  $(LATEXOPTS) $(ARXIVMAINTEX) > /dev/null                 && \
	$(LATEX)  $(LATEXOPTS) $(ARXIVMAINTEX) > /dev/null                 && \
	$(LATEX)  $(LATEXOPTS) $(ARXIVMAINTEX) > /dev/null                 && \
	cd $(TOP)                                                          && \
	echo "Done."                                                       || \
	(less $(BLDDIR)/$(ARXIVNAME).log                                   && \
	echo -e "\n** Log file: $(BLDDIR)/$(ARXIVNAME).log"                && \
	/bin/false)

blddirexist: 
	@[ ! -d $(BLDDIR) ]                 && \
	mkdir $(BLDDIR)                     || \
	/bin/true

outdirexist: 
	@[ ! -d $(OUTDIR) ]                 && \
	mkdir $(OUTDIR)                     || \
	/bin/true

# Tarball targets
alltar: arxivtar
	@echo "Done."

arxivtar:
	@tar zcvf $(ARXIVTGZ) $(ARXIVRELMAKEFILE) $(ARXIVRELSOURCES) $(RELEPSDIR)/*.eps

# Maintenance targets

clean: arxivclean texclean
	rmdir $(BLDDIR)

texclean: arxivtexclean

# ARXIV clean
arxivclean: arxivtexclean
	/bin/rm -f                  \
	   $(OUTDIR)/$(ARXIVPDFOUT) \
	   $(OUTDIR)/$(ARXIVPSOUT)  

arxivtexclean:
	/bin/rm -f                  \
	   $(BLDDIR)/$(ARXIVDVIOUT) \
	   $(BLDDIR)/$(ARXIVAUX)    \
	   $(BLDDIR)/$(ARXIVLOG)    \
	   $(BLDDIR)/$(ARXIVTOC)    \
	   $(BLDDIR)/$(ARXIVFIG)    \
	   $(BLDDIR)/$(ARXIVTAB)    \
	   $(BLDDIR)/*.tex          \
	   $(BLDDIR)/*.eps          \
	   $(BLDDIR)/$(ARXIVNAME).* \
	   $(BLDDIR)/*.bib          \
	   $(BLDDIR)/*~

help:
	@echo
	@echo "Usage: make {clean|texclean|help}"
	@echo "   No arguments:    Build the PDF version of the paper"
	@echo "   clean:           Remove everything that we generate"
	@echo "   texclean:        Remove everything that TeX generates"
	@echo "   help:            This help"
	@echo

